Speed limits in traffic emission models using multi-objective optimization

Climate change compels a reduction of greenhouse gas emissions, yet vehicular traffic still contributes significantly to the emission of air pollutants. Hence, in this paper we focus on the optimization of traffic flow while simultaneously minimizing air pollution using speed limits as controllable parameters. We introduce a framework of traffic emission models to simulate the traffic dynamic as well as the production and spread of air pollutants. We formulate a multi-objective optimization problem for the optimization of multiple aspects of vehicular traffic. The results show that multi-objective optimization can be a valuable tool in traffic emission modeling as it allows to find optimal compromises between ecological and economic objectives.

==> answer_letter.tex <==
	%======================================================================================
	% Responses to reviewers
	
		
\section*{Response to Referee 1 for the Optimization and Engineering submission "Speed limits in traffic emission models using multi-objective optimization"}

We like to thank Referee 1 for carefully reading the manuscript and providing us with helpful comments. This revision tries to address each of those suggestions. Based on the comments and the suggestions made by the Referee, we revised the paper thoroughly and improved the minor revisions. 
All questions/comments are replied below. 


 \begin{enumerate}
     \item \textit{"In the Introduction, the authors say that the optimization of the economic and the environmental aspects “has only been considered separately so far”. This is not exactly true, since both aspects have been considered in a joint manner previously by using multi-objective optimization. They should comment the paper of Vázquez-Méndez et al. [1] where the authors analyse the problem of optimizing the economic aspect (minimal travel time and maximal outflow) simultaneously to the environmental aspect (minimal pollutant concentration), within a multi-objective cooperative framework (that is, computing a Pareto front, similarly to the authors of this paper), where the control are the characteristics of the road junctions (preferences of drivers, ingoing capacities of roads). They should also comment the more recent paper of García-Chan et al. [2] where this problem is addressed from a multi-objective non-cooperative viewpoint (that is, using a hierarchical bi-level Stackelberg strategy)."}

     We thank the referee for the valuable suggestion of the additional literature and included it to our literature overview.

     \item \textit{"With respect of the dispersion model, to be realistic, in equation (3.4a) I miss a term corresponding to a reaction term (of the type $ + \kappa \phi $) where $\kappa$ represents the decay rate for chemical/physical interactions of the pollutant with air or other substances, or even precipitation. This term, if not included, should be at least commented."}

    We included the reaction term \( + \kappa \phi\) to the model description and consequently changed the adjoint equation and its discritization accordingly. We also changed the former parameter \( \kappa\) describing the emission of idling cars to \( \omega\) to maintain a consistent notation. Additionally, we rerun the numerical experiments to analyze the effect of \( \kappa > 0\) to the optimal solution.  
    
    We solved the optimization problem for \( \kappa \in \{0, 0.01, 0.05, 0.1, 1\}\) and displayed the resulting Pareto fronts in \cref{fig: influence kappa}. One can observe that the larger \( \kappa\), the larger the pollution. Furthermore, in case the pollution of idle traffic is also taken into account, the Pareto front follows a linear function the larger \( \kappa\) gets.
    %
     \begin{figure}[ht]
    	\centering
    	\begin{subfigure}[t]{.48\textwidth}
    		\centering
    		\includegraphics[width=\textwidth]{./tikz_revision/front_without_queue_kappa}
    		\subcaption{\(	\min_{\V} \, (-\J_\flow^h(\V), \J_\poll^h(\V \,; 0)) \)}
    		\label{fig: influence kappa no queue}
    	\end{subfigure} \hfill
    	\begin{subfigure}[t]{.48\textwidth}
    		\centering
    			\includegraphics[width=\textwidth]{./tikz_revision/front_with_queue_kappa}
    		\subcaption{\(	\min_{\V} \, (-\J_\flow^h(\V), \J_\poll^h(\V \,; 1/2)) \)}
    		\label{fig: influecene kappa with queue}
    	\end{subfigure}
    	\caption{Influence of \( \kappa\) on the Pareto fronts.}
    	\label{fig: influence kappa}
    \end{figure}
    
    To showcase the influence of \( \kappa\) on the optimal speed limits, we display the range of the optimal speed limits of the optimization problem \(	\min_{\V} \, (-\J_\flow^h(\V), \J_\poll^h(\V \,; 1/2)) \) for \( \kappa \in \{0.1, 1\} \) in \cref{fig: speed kappa}. Notice, that in the formulation of the optimization problem, the pollution of idle vehicles waiting in the queue is taken into account.
       
    The optimal speed limits for these two cases look overall very similar. However, there are three differences that are easy to spot. 
    \begin{enumerate}[label=(\roman*)]
    	\item The minimal optimal speed limit on road \( e = 1\) is \( V_1^{\max} \approx 1\) for \( \kappa = 0.1\) compared to \( V_1^{\max} \approx 1.4\) for \( \kappa = 1\).
    	\item A similar effect is seen on road \( e = 2\), where the minimal, optimal speed limit is is \( V_2^{\max} = 0.25\) for \( \kappa = 0.1\) compared to \( V_2^{\max} \approx 5\) for \( \kappa = 1\).
    	\item Finally, on road \( e = 3\), the maximal optimal speed limit reduces from \( V_3^{\max} = 2\) to \(V_3^{\max} \approx 1.8\).
    \end{enumerate}
    The extinction rate \( \kappa\) has a similar effect on the optimal speed limits of the problem \(	\min_{\V} \, (-\J_\flow^h(\V), \J_\poll^h(\V \,; 0)) \), i.e., idle traffic does not emit pollutants in this scenario. Hence, we omit further images here.
    
     \begin{figure}[ht]
    	\centering
    	\begin{subfigure}[t]{.48\textwidth}
    		\centering
    		\includegraphics[width=\textwidth]{./tikz_revision/speed_limit_with_queue_kappa01}
    		\subcaption{\(	\kappa = 0.1 \)}
    		\label{fig: speed kappa 01}
    	\end{subfigure} \hfill
    	\begin{subfigure}[t]{.48\textwidth}
    		\centering
    		\includegraphics[width=\textwidth]{./tikz_revision/speed_limit_with_queue_kappa1}
    		\subcaption{\( \kappa = 1 \)}
    		\label{fig: speed kappa 1}
    	\end{subfigure}
    	\caption{Influence of \( \kappa\) on the optimal speed limits when the pollution of idle traffic is taken into account.}
    	\label{fig: speed kappa}
    \end{figure}
    
   
    
    Also note that the CFL condition cited in Remark 5.2 is no longer valid for \( \kappa > 0\) as it requires \( \kappa = 0\). However, we found for our testing cases it was sufficient to set the temporal step size to \( \frac{1}{3} \Delta t_{\rm CFL}\) where \( \Delta t_{\rm CFL}\) satisfies the old CFL condition, in order to maintain stability of our numerical scheme. We extended Remark 5.2 by this comment too.
         

     \item \textit{"Also in the same subsection, for boundary condition (3.4c), this is a null Dirichlet condition that fixes the value of pollutant concentration to zero, but that does not imply “that pollutant cannot enter the domain from outside”, as the authors say. This boundary condition could be true maybe for the case of non-diffusion ($ \mu = 0 $), but not in the case presented by the authors. Another type of boundary should be used, for instance, that one presented in the work of Parra-Guevara \& Skiba [3]. Any change in equation or boundary conditions here, would change also the adjoint equation (4.6)."}
     
     We changed the Dirichlet boundary condition to the suggested one to be consistent with the existing literature, i.e., \cite{Alvarez2017,Alvarez2018,Parra2003}. Hence, we also rerun the numerical experiments. 
     
     \begin{figure}[ht]
     	\centering
     	\begin{subfigure}[t]{.45\textwidth}
     		\centering
     		\input{./tikz/pareto_front_without_queue}
     		\subcaption{Dirichlet boundary conditions.}
     		\label{fig: dirichlet}
     	\end{subfigure} \hfill
     	\begin{subfigure}[t]{.45\textwidth}
     		\centering
     		\input{./tikz_revision/pareto_front_without_queue_review}
     		\subcaption{Robin boundary conditions (as suggested).}
     		\label{fig: robin}
     	\end{subfigure}
     	\caption{Comparison of the Pareto front of \(  	\min_{\V} \, (-\J_\flow^h(\V), \J_\poll^h(\V \,; 0))  \) for different types of boundary conditions on the inflow boundary.}
     	\label{fig: new boundary conditions}
     \end{figure}
     
     \begin{figure}[ht]
    	\centering
    	\begin{subfigure}[t]{.45\textwidth}
    		\centering
    		\input{./tikz/speed_limit_range_without_queue}
    		\subcaption{Dirichlet boundary conditions.}
    		%\label{fig: dirichlet}
    	\end{subfigure} \hfill
    	\begin{subfigure}[t]{.45\textwidth}
    		\centering
    		\input{./tikz_revision/speed_limit_range_without_queue_review}
    		\subcaption{Robin boundary conditions (as suggested).}
    		%\label{fig: robin}
    	\end{subfigure}
    	\caption{Comparison of the optimal speed limits of \( 	\min_{\V} \, (-\J_\flow^h(\V), \J_\poll^h(\V \,; 0))  \) for different types of boundary conditions on the inflow boundary.}
    	\label{fig: new boundary conditions speed}
    \end{figure}
     
     In \cref{fig: new boundary conditions}, we analyze the influence of the boundary condition on the inflow boundary, on the optimal solution of the optimization problem
     \begin{equation*}
     	\min_{\V} \, (-\J_\flow^h(\V), \J_\poll^h(\V \,; 0)) 
     \end{equation*}
     In \cref{fig: dirichlet} we set Dirichlet boundary conditions on the inflow boundary, and in \cref{fig: robin} we set Robin boundary conditions as suggested by the referee. We observe, that the change of the boundary conditions has no visible effect on the solution for our example.  In \cref{fig: new boundary conditions speed}, we also visualized the corresponding optimal speed limits, observing the same effect.     
     The slight difference between these two solutions are most likely due to the solving algorithm as it is based on a pattern search which uses (random) sampling.
     We omit a visualization of the comparison for the optimization problem \(\min_{\V} \, (-\J_\flow^h(\V), \J_\poll^h(\V \,; 1/2)) \), where idling vehicles are taken into account, because the influence is, again, barely visible.     
     
     


    \item \textit{"Fig. 9(b) could be confusing for readers, since they could understand that speed limits vary linearly (and they are constants). I suggest the authors to use only the dots (like in Fig. 10(b)) or to use piecewise constant lines."}  

    We removed the connecting line between to speed limits in (now) \cref{fig: speed limit routes without queue} to avoid confusion.
 \end{enumerate}
	
	
	
\section*{Response to Referee 2 for the Optimization and Engineering submission "Speed limits in traffic emission models using multi-objective optimization"}

We like to thank Referee 2 for carefully reading the manuscript and providing us with helpful comments. This revision tries to address each of those suggestions. Based on the comments and the suggestions made by the Referee, we revised the paper thoroughly and improved the minor revisions. 
All questions/comments are replied below. 

\begin{enumerate}
    \item \textit{"Page 3, line 13 from above: ‘...away form the node’ \(\rightarrow\) ‘...away from the node’."}
    
    We corrected the typo.
    
    \item \textit{"Page 3, line 3 from below: Problem (2.1) is well-posed, if we also add boundary conditions"}

    We included the remark.
    
    \item \textit{"Page 4, line 2 from below: ‘For a in-depth and...’ \(\rightarrow\) ‘For an in-depth and...’"}

    We corrected the typo.
    
    \item \textit{"Page 10, formula (4.4): Might it also be meaningful to consider \(\J_\diff\) and \(\J_\queue\) as two different objectives so that the cost functional has three components (instead of two)?"}

    We thank the referee for this valuable comment. We computed the Pareto front for cost functional consisting of the functions \( (\J_\flow, \J_\diff, \J_\queue)\) and compared the results with the already existing ones. The numerical experiments were extended by this comparison which can now be found in \cref{fig: coordinates without queue,fig: coordinates with queue,fig: composition}.
    
    \item \textit{"Page 13, line 6 from above: I guess you should write ’...at the end of the exit roads...’ instead of ‘...at the end of exist roads...’."}

    We included the missing "the".
    
    \item \textit{"Page 14, line 14 from above: Where have you introduced the wind field?Is this the field v in (3.4a)? Maybe I have overseen that. Furthermore: ‘...diffusion coefficent...’ \(\rightarrow\) ‘...diffusion coefficient...’"}

    The referee is correct. The wind field mentioned in Remark 5.2 is the same one as in equation (3.4a). It was introduced at the beginning of Section 3.2.
    We included a reference to equation (3.4) to avoid any confusion and corrected the typo that was pointed out.

    
    \item \textit{"Page 16, line 1 from below: Please add information regarding the optimization method used by Matlab’s Optimization Toolbox"}

    We added additional information on the method used by Matlab's Optimization Toolbox.
    
    \item \textit{"Page 22, Section 7: There are results available for multi-objective optimization problems governed by elliptic or parabolic partial differential equations, but – up to my knowledge – there are no mathematical investigations for multi-objective optimization problems governed by hyperbolic PDEs. This is definitely also an interesting (and important) research field for the future"}
    
    We thank the referee for the insightful comment. The focus of the paper lies on the modeling and simulation of the problem. However, it would be great to have theoretical results that, for example, provide the existence of a solution to the proposed multi-objective optimization problem.

\end{enumerate}

\section*{Further Updates in the Revised Paper}
\begin{itemize}
	\item We corrected the description of the discretization of the time-reversed adjoint's advection term. Before we dicretized \( \vv \cdot \nabla \p(\x,t)\) with the Upwind scheme. However, the full term is \( - \vv \cdot \nabla \p(\x,t)\). Neglecting the sign, leads to an incorrect discretization. Notice, that the actual implementation in the experiments was correct. Hence, this was only a notation error.
%	\item Added plot with normal and log axis for last experiment
\end{itemize}
	

==> tex/outline.tex <==
\section{Outline}
\subsection{Introduction/Storyline}
\begin{itemize}
    \item Earth dies also because air pollutants harm environment (soil, health, climate) leads to chain recation causing
        further damage. Vehicular traffic emits a variaty of air pollultants, and thus, contributation to destruction of our planet. Still, 
        vehicular traffic makes upto \( 75 \%\) of travelled kilometers in Germany \( \rightarrow\) encouter vehicular traffic 
        daily (in one form or another)
    \item \textbf{Goal:} make vehicular traffic as convient/comforable as possible, e.g. short travel times, less congestion.       But moving to mars seems not like an option so reduce environmental impact. As we are greedy we aim for both! 
    \item \textbf{Idea:} Optimize both objectives simultaneously but not by adding both objectives. Instead really try to optimize both individually \( \rightarrow \) multi-objective (also multi-criteria, vector-valued) optimization.
    \item \textcolor{teal}{\textbf{Focus} on the idea to combine traffic emission modeling with multi-objective optimization
        rather on the implementational details/details on the individual models as those are well-know.}
\end{itemize}


\subsection{Traffic Model}
\begin{itemize}
    \item Model traffic based on traffic density (but why tho?) on a road network.
    \item Make speed-limit dependence clear (!) by choosing the right (or very basic) flux function of the Greenshield model.
    \item Need to model queues if we include queue length in computation of total emission. What about junctions in general        (here maybe citations only)? 
\end{itemize}

\subsection{Emission Model}
\begin{itemize}
    \item Models the emission of air pollutants due to vehicular traffic by the emission rate 
    \item Estimation is based on properties the traffic model provides. Essential because speed-limit-dependence.
    \item Why we extend the emission to a set of positive Lebesgue-measure and how.
\end{itemize}

\subsection{Disperison Model}
\begin{itemize}
    \item Yields concentration of air pollutant(s) over time \( \rightarrow \) dynamic is influenced by wind and diffusion, also maybe chemical reactions in air because we do not live in a vacuum. 
    \item Model also for production of air pollutatant(s) due to vehicular traffic. (Very crucial -- let's say even essential --
        because the source term connects the emission of air pollutants due to vehicular traffic with the spread of the initial
        distribution of air pollutant(s). Also speed-limit-dependence)
    \item Why is this property of interest? High concentration of air pollutants are associated with poor amibent air quality
        and may become hazardous!
\end{itemize}

\subsection{Optimization}
\begin{itemize}
    \item How do we define \emph{optimality} in case of multiple objective/vector-values objectives? 
    \item What are the \emph{mathematically rigourous} objectives? How do we quantify desired prooperties by a scalar value?
    \item We can rewrite the ecological objectives with the adjoint (citation only?)
\end{itemize}

\subsection{Numerics}
\begin{itemize}
    \item Cite standard literature for numerical schemes, do not cover treatment of boundary conditions of dispersion model (or only very vaguely? What about junctions?)
    \item Need equations of numerical schemes to know discrete variables, BUT numerical properties are irrelevant.
    \item Give discrete counterparts of discrete equations as we cannot solve involved PDEs explicitly
        \( \rightarrow \) Solve discrete problem instead!
\end{itemize}

\subsection{Experiments}
\begin{itemize}
    \item Results: Objectives to minimize environmental impact and maximize accumulated traffic flow are conflicting
         \( \rightarrow \) plots of Pareto front (What are suitable/realistic parameters for \(\kappa\)?)
\end{itemize}

\subsection{Outlook}
\begin{itemize}
    \item More advanced emission model \( \rightarrow\) replace first with second-order model (GRAZ).
    \item Validate with real data.
    \item Combine with integer programming, 
    \item Extract only a single (or a few \( \approx (2-5)\)) optimal solutions.
\end{itemize}

\subsection{Left Overs}
\begin{itemize}
    \item Why are line integrals combined with the adjoint admissable? 
    \item Unit of emission rate and concentration / time have to be equal!
    \item What about the existence of solutions in dependence of the speed-limit policy? How can we shorten the proofs and necessary definitions? Only citations?
    \item Shorted definition and notation of road networks, junctions, etc.
    \item Paramters for the experiments.
\end{itemize}


